The Stagger Code for Accurate and Efficient, Radiation-Coupled MHD Simulations

We describe the Stagger Code for simulations of magneto-hydrodynamic (MHD) systems. This is a modular code with a variety of physics modules that will let the user run simulations of deep stellar atmospheres, sunspot formation, stellar chromospheres and coronae, proto-stellar disks, star formation from giant molecular clouds and even galaxy formation. The Stagger Code is efficiently and highly parallelizable, enabling such simulations with large ranges of both spatial and temporal scales. We, describe the methodology of the code, and present the most important of the physics modules, as well as its input and output variables. We show results of a number of standard MHD tests to enable comparison with other, similar codes. In addition, we provide an overview of tests that have been carried out against solar observations, ranging from spectral line shapes, spectral flux distribution, limb darkening, intensity and velocity distributions of granulation, to seismic power-spectra and the excitation of p modes. The Stagger Code has proven to be a high fidelity code with a large range of uses.

==> EOS.tex <==

Simple equations of state, e.g. H and He-only ideal gas, are calculated analytically
on the fly as needed.  More complex equations of state 
are interpolated from a table as a function of log density and internal energy per unit mass.

%++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
\subsection{Table Structure}
%++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
\label{sect:tablestructure}

The equation of state (EOS) table contains {\tt Ntbvar}$\ge 6$ rectangular arrays of
gas pressure $\ln P_{\rm gas}$, Rosseland mean opacity, $\ln\kappa_{\rm Ross}$,
temperature, $\ln T$, electron number density, $n_e$, 
Planck mean opacity, $\ln\kappa_{\rm Planck}$ and the
monochromatic opacity at 5\,000\,{\AA}, $\ln\kappa_{5000}$. Other variables
can be added at the end.  An older table format included the binned opacities 

These variables are functions of a regular grid of density, $\ln\rho$, and
internal energy per mass, $\ln e$. The extent and resolution of the grid is given
in the header of the table, together with the number of elements and their
abundances used in the calculation, the option flags that were set for the
calculation and the revisions of the codes used in the calculation, as well as
date- and time-stamps, uniquely identifying the table.

Convective stability, particularly in deep layers where the velocities and
entropy fluctuations are very small, are sensitive to errors in the EOS, so 
bicubic interpolation in the tables is used. 
Each of the {\tt Ntbvar} table entries, $f$, are accompanied by their partial
derivatives, $\dxdy{f}{\ln e}\Delta\ln e$ and $\dxdy{f}{\ln\rho}\Delta\ln\rho$,
to facilitate this higher order interpolation.

The opacity calculations do not provide derivatives so they have to be evaluated
numerically. We do so by computing opacities at two guide points at
$\pm\Delta\ln e/3$ from the table point (and inverted to $\log_{10}T$ with the
same function as above), giving second-order derivatives, and similarly for
$\pm\Delta\ln\rho /3$, providing smooth interpolations in the tables. 

The presence of Rosseland mean opacity and $\kappa_{5000}$ opacity in this table 
is for convenience in subsequent
analysis of the simulations, e.g. for evaluating the Rosseland optical depth scale.

%++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
\subsection{Stellar Atmospheres}
%++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
\label{sect:StarAtm_ExpRemoEOS}

The thermodynamics is supplied by the Mihalas-Hummer-D{\"a}ppen (MHD) EOS
\citep{mhd1,mhd2} custom computed for 15 element mixtures by
\citet{trampedach:T-tau}. These are computed as function of $\log_{10}T$ and
$\log_{10}\rho$, and need to be inverted from $\log_{10}T$ to $\ln e$, the
independent variable of the Stagger simulations. This is done by exploiting the
analytical partial derivatives of the MHD EOS, that allows for an accurate
and physical third-order interpolation to a new regular $\ln e$-grid, and with
analytical and consistent $\ln e$-derivatives.

The EOS tables are \emph{universal} in the sense that they are
applicable to any simulation with the given composition. Therefore we choose a
large extent of these table, to encompass most stellar atmospheres, with a
default of $\log_{10}\rho=[-14;0]$, $\log_{10}e=[11;14]$, and a resolution of
$N_e=300$ and $N_\rho=57$. The latter is dictated by the original MHD EOS
calculation, which typically use $\Delta\rho=0.25$.




==> defs_backup.tex <==
\newcommand{\svec}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\nts}{\negthinspace}
\newcommand{\stimes}{{\kern-0.08em\times\kern-0.1em}}
\newcommand{\ednote}[1][]{{\newline\scriptsize\bf[#1 -]}}
%!TEX encoding = UTF-8 Unicode
%  Miscellaneous equation macros
%
\newcommand{\eb}[1]{\begin{equation}\label{eq:#1}}
\newcommand{\en}{\end{equation}}
\newcommand{\eab}[1]{\begin{eqnarray}\label{eq:#1}}
\newcommand{\ean}{\end{eqnarray}}
\newcommand{\Eq}[1]{Equation~\ref{eq:#1}}


\newcommand{\Eqs}[2]{Equations~\ref{eq:#1}--\ref{eq:#2}}
\newcommand{\Fig}[1]{{Figure~\ref{fig:#1}}}
\newcommand{\Section}[1]{Section~\ref{sect:#1}}
\newcommand{\Table}[1]{Table~\ref{table:#1}}

\newcommand{\grad}{\nabla}
\newcommand{\curl}{\nabla\times}
\newcommand{\ddt}[1]{\frac{\partial #1}{\partial t}}
\newcommand{\ddx}[1]{\frac{\partial #1}{\partial x}}
\newcommand{\ddy}[1]{\frac{\partial #1}{\partial y}}
\newcommand{\ddz}[1]{\frac{\partial #1}{\partial z}}
\newcommand{\ddi}[1]{\frac{\partial #1}{\partial x_i}}
\newcommand{\ddj}[1]{\frac{\partial #1}{\partial x_j}}
\newcommand{\DDt}[1]{\frac{D #1}{D t}}
%\newcommand{\ddt}[1]{{\partial #1/\partial t}}
%\newcommand{\ddx}[1]{{\partial #1/\partial x}}
%\newcommand{\ddy}[1]{{\partial #1/\partial y}}
%\newcommand{\ddz}[1]{{\partial #1/\partial z}}
%\newcommand{\ddi}[1]{{\partial #1/\partial x_i}}
%\newcommand{\ddj}[1]{{\partial #1/\partial x_j}}
%\newcommand{\DDt}[1]{{D #1/ D t}}
%
%  Introduce boldface math-italics - invoked with, e.g., \vec{F}
%
\DeclareMathAlphabet{\mathbfit}{OML}{cmm}{b}{it}
\renewcommand{\vec}[1]{\mathbfit{#1}}

\renewcommand{\div}{\nabla\cdot}
\renewcommand{\d}{{\rm d}}
\newcommand{\dd} [2]{{\frac{{\rm d}{#1}}{{\rm d}{#2}}}}
\newcommand{\bin}{{\{\lambda\}_i}}

\newcommand{\uu}{\vec{u}}
\newcommand{\ux}{u_{\rm x}}
\newcommand{\uy}{u_{\rm y}}
\newcommand{\uz}{u_{\rm z}}
\newcommand{\gz}{g_{\rm z}}
\newcommand{\Hp}{H_{\rm P}}
\newcommand{\rr}{\vec{r}}
\newcommand{\Om}{\vec{\Omega}}
\newcommand{\Frad}{\vec{F}_{\rm rad}}
\newcommand{\Qrad}{Q_{\rm rad}}
\newcommand{\Qvisc}{Q_{\rm visc}}
\newcommand{\Tvisc}{\vec{\tau}_{\rm visc}}
\newcommand{\Tij}{\tau_{ij}}
\newcommand{\sij}{s_{ij}}
%
%  Radiative quantities
\newcommand{\Bv}{B_{\nu}}
\newcommand{\Bl}{B_{\lambda}}
\newcommand{\Sv}{S_{\nu}}
\newcommand{\Sl}{S_{\lambda}}
\newcommand{\Iv}{I_{\nu}}
\newcommand{\Il}{I_{\lambda}}
\newcommand{\Jl}{J_{\lambda}}
\newcommand{\tauv}{\tau_{\nu}}
\newcommand{\taul}{\tau_{\lambda}}
\newcommand{\kv}{\kappa_{\nu}}
\newcommand{\kl}{\kappa_{\lambda}}
\newcommand{\sigl}{\sigma_{\lambda}}
\newcommand{\al}{a_{\lambda}}
%
%  Energies and fluxes
\newcommand{\Ekin}{E_{\rm kin}}
\newcommand{\Etherm}{E}
\newcommand{\Fconv}{\vec{F}_{\rm conv}}
\newcommand{\Fvisc}{\vec{F}_{\rm visc}}
\newcommand{\Fkin}{\vec{F}_{\rm kin}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\lbc}{{\rm bot}}
\newcommand{\BB}{\vec{B}}
\newcommand{\EE}{\vec{E}}
\newcommand{\JJ}{\vec{J}}
\newcommand{\grav}{\vec{g}}
\newcommand{\dxdycz}[3]{\left( \frac{ \partial #1 }{ \partial #2 }\right)_{#3}}
\newcommand{\dxdy}[2]{\frac{ \partial #1 }{ \partial #2 }}
\newcommand{\mfrac}[2]{{\textstyle{\frac{#1}{#2}}}}
%  Boldface vectors
%
\newcommand{\bvec}[1]{\boldsymbol{#1}}
%
%  Use italic foreign abbreviations
%
\newcommand{\etal}{\it et al.}
\newcommand{\eg}  {\it e.g.}        % exempli gratia {f.eks.}
\newcommand{\cf}  {\it cf.}         % confer {jvnf.}
\newcommand{\ie}  {\it i.e.}        % id est {d.v.s.}
\newcommand{\etc} {\it etc.}
\newcommand{\viz} {\it viz.}        % videlicet {namely}
%
%  Double the linespacing in equation arrays
%
\setlength{\jot}{6pt}
%\the\arraycolsep
\setlength{\arraycolsep}{1.5pt}
%
%  Macro to set equations in an array numbered alphabetically.
%    It doesn't work to \renewcommand{\theequation}{\theorigeqn}.
%    Use the \let-construction instead (both places).
%
\newcounter{saveeqn}
\newcounter{temp}
%                                     saveeqn = equation
\newcommand{\alpheqn}{\setcounter{saveeqn}{\value{equation}}%
%       saveeqn = saveeqn + 1,     equation = 0,   save the original def.
  \stepcounter{saveeqn}\setcounter{equation}{0}\let\theorigeqn=\theequation%
%    New def. of theequation:                temp = equation
  \renewcommand{\theequation}{\setcounter{temp}{\value{equation}}%
%                     equation = saveeqn,  use the original \theequation def.
    \setcounter{equation}{\value{saveeqn}}\theorigeqn%
%                     equation = temp      a,b,c,d,...
    \setcounter{equation}{\value{temp}}\alph{equation}}}
%    Reset after using \alpheqn
\newcommand{\reseteqn}{\setcounter{equation}{\value{saveeqn}}
  \let\theequation=\theorigeqn}
%
%  Various equation styles, all with the label as argument.
%
\newcommand{\be}[1]{\begin{equation}\label{#1}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}[1]{\begin{eqnarray}\label{#1}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beaa}[1]{\alpheqn\begin{eqnarray}\label{#1}}
\newcommand{\eeaa}{\end{eqnarray}\reseteqn}
\newcommand{\mideqn}{\nonumber\\[-2\jot] &{\vbox{\hsize=0pt}}&
	\nonumber\\[-1.25\baselineskip] &{\vbox{\hsize=0em}}&\\[-0.75\baselineskip]}
\newcommand{\gwig}{{\leavevmode\kern0.3em\raise.3ex\hbox{$>$}
                    \kern-0.8em\lower.7ex \hbox{$\sim$}\kern0.3em}}
\newcommand{\lwig}{{\leavevmode\kern0.3em\raise.3ex\hbox{$<$}
                    \kern-0.8em\lower.7ex \hbox{$\sim$}\kern0.3em}}
%
%  User-friendly macro for including PS figures.
\newcommand{\mfigcap}[2]{\figcaption{#2\label{#1}}}
\newcommand{\figdir}{figs}
\newcommand{\mfigur}[3]
    {\begin{figure}[htb]
        \centerline{\includegraphics[height=#2,clip=true]{\figdir/#1.jpg}}
%       \centerline{\includegraphics[height=#2,clip=true]{\figdir/#1.ps}}
        \caption{\label{fig:#1}#3}
    \end{figure}}
\renewcommand{\floatpagefraction}{.95}
\renewcommand{\topfraction}{.9}
\renewcommand{\bottomfraction}{1.}
\renewcommand{\textfraction}{.1}
%
%  An easy-to-use macro for making A&A-style tables
%
\def\aatab#1#2#3#4#5#6{\ifthenelse{\equal{*}{#1}}
{\begin{table*}[htbp]\caption{\label{#2} #3}
    \centering
    \begin{tabular}{#4}
      \hline\noalign{\smallskip} #5
          \noalign{\smallskip} \hline \noalign{\smallskip} #6
          \noalign{\smallskip} \hline
        \end{tabular}
\end{table*}}
{\begin{table}[htbp]\caption{\label{#1} #2} 
    \centering
    \begin{tabular}{#3}
      \hline\noalign{\smallskip} #4
      \noalign{\smallskip} \hline \noalign{\smallskip} #5
      \noalign{\smallskip} \hline
    \end{tabular}
\end{table}}}
\newcommand{\oh}[1]{\omit\hidewidth #1\hidewidth}


==> dissipation.tex <==

\subsection*{Alternative 2}
Absorb the factor of 2 into the definition of $\nu_{ij}$:
\begin{equation}
{\partial (\rho u_i) \over \partial t}
= {\partial\over\partial x_j} \left( \rho \nu_{ij} S_{ij} \right)
= {\partial\over\partial x_j} \left( \tau_{ij} \right)
\end{equation}

\begin{equation}
S_{ij} = \frac{1}{2} ({\partial u_i \over \partial x_j} + {\partial u_j \over \partial x_i})
\end{equation}

\begin{eqnarray}
{\partial \over \partial t} (\Sigma_{i} \frac{1}{2}\rho u_i^2)
& = & {\Sigma_{i} u_i \partial (\rho u_i) \over \partial t} + ...
\\ & = & \Sigma_{ij} u_i {\partial\over\partial x_j}
 \left( \rho \nu_{ij} S_{ij} \right)
\\ & = & \Sigma_{ij}{\partial u_i \over\partial x_j}
 \left( \rho \nu_{ij} S_{ij} \right) + ...
\\ & = & \Sigma_{ij}
 \rho \nu_{ij} S_{ij}^2 + ...
 = \Sigma_{ij} \tau_{ij} S_{ij}
\end{eqnarray}

\section*{Smagorinsky viscosity}
The Smagorinsky viscosity is implemented e.g. in the {\tt pde\_omp\_nud.f90} version of the PDE routines,
where it is defined such that it contributes an additional
\begin{equation}
\nu_{ij} = ... + \Delta x_{ij} C_{\rm smag} \sqrt{2 (\sum_m S_{mm}^2 + 2 \sum_{m < n} S_{mn}^2)} ,
\end{equation}
where the strain rate tensor is defined as
\begin{equation}
S_{ij} = \frac{1}{2} ({\partial u_i \over \partial x_j} + {\partial u_j \over \partial x_i}) ,
\end{equation}
and the symmetrized grid spacing, $\Delta x_{ij}$, is defined as
\begin{equation}
\Delta x_{ij} = \frac{1}{2} (\Delta x_i + \Delta x_j) .
\end{equation}
It might be better to define the symmetrized grid spacing, $\Delta x_{ij}$, as
a geometric mean,
\begin{equation}
\Delta x_{ij} = (\Delta x_i \Delta x_j)^\frac{1}{2} ,
\end{equation}
or
a harmonic mean,
\begin{equation}
\Delta x_{ij} = 2\Delta x_i \Delta x_j/(\Delta x_i + \Delta x_j) ,
\end{equation}
to avoid too large diffusive effects from off-diagonal terms.

\vspace{6pt}\noindent
The $\nu_{ij}$ definition is equivalent to
\begin{equation}
\nu_{ij} = ... + \sqrt{2} \Delta x_{ij} C_{\rm smag} \sqrt{\sum_{mn} S_{mn}^2} ,
\end{equation}
so it is properly cylindrically symmetric for vortex type flows.



==> io_old.tex <==
Data for stagger is input via a file of namelists of input parameters.  
The namelists are read in the order: io, run, var, grid, pde which are read in the
routine params.f90.  Then come: bdry (in BOUNDARIES/boundary routine), slice
(slice.f90), quench (STAGGER/quench.f90), eqofst (EOS/eos routine), part
particles.f90), force (FORCING/gravity or forcing routine), 
init (INITIAl/initialization routine), expl (FORCING/noexplode or stars or sn), 
and cool (COOL/radiation or cooling routine).  Default values are specified in 
the routines that
read each namelist.  If the parameters in a given namelist are not needed it can be
left blank.  In addition there are some initialization routines that may or may not
be compiled into the executable that have additional namelist inputs.

The namelists, in the order they are read, are:

\begin{center}
{\Large Namelist io}
\begin{tabular}{|l|l|c|c|c|}
\hline
name & description & default & atmosphere sun & turbulence  \\
\hline
from & name input snapshot file & & & \\
\hline
file & name output snapshot file & & &  \\
\hline
iread & snapshot number to read & & & \\
      & iread = -1 do not read snapshot & & & \\
\hline
iwrite & snapshot number to write & & & \\
\hline
nsnap & write snapshot every nsnap steps & 20 & & \\
\hline
tsnap & write snapshot every tsnap time & 0 & & \\
\hline
nscr & overwrite scr file ever nscr steps & 10 & & \\
\hline
tscr & overwrite scr file every tscr time & 0 & & \\
\hline
nstep & maximum time steps in run& 9999999 & & \\
\hline
tstop & maximum time of run & 999999, & & \\
\hline
do\_scp & & false & t & \\
\hline
scp\_dir & & & & \\
\hline
do\_subdir & & false & & \\
\hline
do\_master\_io & & false & t & \\
\hline
do\_parallel\_io & & false & t & \\
\hline
do\_single & & \\
\hline
do\_init\_smooth & & false & & \\
\hline
do\_init\_smooth\_hd & & false & & \\
\hline
do\_divb\_clean & clean initial div(B) & false & t & \\
\hline
divb\_iter & maximum cleaning itterations & 15 & & \\
\hline
divb\_eps & cleaning accuracy & $10^-4$ & & \\
\hline
do\_concurrent & & false & & \\ 
\hline
nconcurrent & & 0 & & \\
\hline
tconcurrent & & 0 & & \\
\hline

\end{tabular}
\end{center}

\begin{center}
{\Large Namelist run}
\begin{tabular}{|l|l|c|c|c|}
\hline
name & description & default & atmosphere sun & turbulence  \\
\hline
t & initial time & 0 & & \\
\hline
dt & initial timestep & 0.0000111 & & \\
\hline
Cdt & Courant condition & 0.5 & 0.4 & 0.3 \\
\hline
Cdtd & Courant condition on viscosity & 0.8 & 0.6 & 0.7 \\
\hline
Cdtr & Courant condition on density \& energy changes  & 0.4 & 0.1 & \\
\hline
timeorder & Time integration order & 3 && \\
\hline
iseed & Random number seed & -77 && -1063256064 \\
\hline
idbg & Debug printout control & 0 && \\
\hline
do\_trace & trace calls & false && \\
\hline
do\_dump & enable dumps & false && \\
\hline
do\_compare & compare results of 2 runs & false && \\
\hline
do\_logcheck & write check info to log file & false & t & \\
\hline
do\_check & write check file & false && \\
\hline 
do\_flags & control execution with flag files & false && \\
\hline 
do\_timer & timer calls & false && \\
\hline 
do\_validate & bitwise reduction precision etc & false && \\
\hline
rank\_timer & for each rank & false && \\
\hline
dbg\_select & select topic for debugging & 0 && \\
\hline
dbg\_baarrier & barrier number to test & 0 && \\
\hline
dbg\_level & & 0 && \\
spin\_barrier & spins to do at barrier & 0 && \\
\hline
t\_prop & proper time, for field upping & 0 && \\
\hline
E\_prop & proper energy, for field upping & 0 && \\
\hline
E\_mag & actual energy & 0 && \\
\hline
check\_barrier & check barriers are in sync & false && \\
\hline
use\_isend & default: use MPI\_Issend & 2 && \\
\hline

\end{tabular}
\end{center}

\begin{center}
{\Large Namelist vars}\\
\begin{tabular}{|l|c|}
\hline
do\_density &  \\ \cline{1-1}
do\_momenta &  \\ \cline{1-1}
do\_energy & specify which equations to include \\ \cline{1-1}
do\_mhd &  \\ \cline{1-1}
do\_pscalar &  \\ 
\hline

\end{tabular}
\end{center}

\begin{center}
{\Large Namelist grid}
\begin{tabular}{|l|l|c|c|c|}
\hline
name & description & default & atmosphere sun & turbulence  \\
\hline
mx,my,mz & dimensions of computational box & 33 && \\
\hline
mpi\_nx,nyknz & dimension of mpi domains & 0 && \\
\hline
sx,sy,sz & physical dimensions of box & 1 && \\
\hline
z,y,zmin & minimum of [xyz]-axis, & 1e6 && \\
         & if [xyz[min=1e6 init\_mesh determins value &&& \\
\hline
lb & lower boundary & 1 && \\
\hline
ub & upper boundary & 0 && \\
\hline
omega,omega{x,y,z} & coordinate system rotation & 0 && \\
\hline
meshfile & file with mesh information & mesh.dat && \\
\hline

\end{tabular}
\end{center}

\begin{center}
{\Large Namelist pde}
\begin{tabular}{|l|l|c|c|c|}
\hline
name & description & default & atmosphere sun & turbulence  \\
\hline
do\_stratified & special treatment of some operations & false && \\
\hline
stratified & subtract average energy & 0 && \\
           & =1 with quench, =2 subtract flux, =3 with quench &&& \\
\hline
do\_loginterp & interpolate in logs & true & t & t \\
\hline
do\_2nddiv & second order divergences & false & t & t \\
\hline
do\_lnpg & gradient of ln(P gas) & false & t & \\
\hline
do\_nodrag & no net viscous drag & true && \\
\hline
do\_kepler & subtract Kepler velocity && \\
\hline
do\_massexact & mass conservation & true && \\
\hline
\do\_max5 & average \& smooth over 5 zones & false && \\
do|max5\_hd & in HD&&& \\
do|max5\_mhd & in MHD&&& \\
\hline
gamma & gas gamma & 1.666667 && 1 \\
\hline
nu1 & normal viscosity & 0.025 & 0.05 & 0.003\\
\hline
nu2 & shock viscosity & 0.5 & 1.5 & 0.3 \\
\hline
nu3 & sound speed cutoff & 0 & 0.05 & 0.003 \\
\hline
nu4 & ln(rho) gradient coefficient & 0 & 1.5 & 1.4 \\
\hline
nuS & solenoidal fraction & & 1 & \\
\hline
nur & relative mass diffusion & 0 && 0.1 \\
\hline
nuE & relative energy diffusion & 1 && \\
\hline
\hline
nuB & relative B diffusion & 1 && \\
\hline
nup & relative passive scalar diffusion & 0.05 && \\
\hline
do\_aniso\_nu & anisotropic nu, for skew aspect ratios & true && \\
\hline
do\_aniso\_eta & anisotropic nu, for skew aspect ratios & true && \\
\hline
d2lnr\_lim & do 2nd order divergence with $d^2 \ln\rho$ larger && 0.3 & \\
\hline
nrho & decrease compressiv viscority for depths > nrho & off && \\
\hline
Csmag & Smagorinsky constant & 0.15 & 0.01 & \\
\hline
Ssmag & Smagorinsky constant & 0.05 && \\
\hline
csound & for polytropic EOS & 1 && \\
\hline
cmax & maximum Alfen speed & 0 & 20 & \\
\hline
do\_massflux & include viscous mass diffusion & false && \\
\hline
t\_Bgrowth & growth rate of B & 0 && \\
\hline
CdivB & limit divB diffusion * < 0.11 & 0.06 & \\
\hline
ambi & ambipolar diffusion & 0 && \\
\hline
nu\_atmos & atmospheric diffusion term && \\
\hline
nu\_inner & inner boundary for atmospheric diffusion & 1.4 && \\
\hline
nu\_outer & outer boundary for atmospheric diffusion & 1.6 && \\
\hline
do\_upping & field upping to keep magnetic energy constant & false && \\
\hline
do\_cylatmos & outer edge for atmospheric diffusion & false && \\
\hline

\end{tabular}
\end{center}

\begin{center}
{\Large Namelist bdry}
\begin{tabular}{|l|l|c|c|c|}
\hline
name & description & default & atmosphere sun & turbulence  \\
\hline
lb & lower boundary & 0 && \\
\hline
ub & upper boundary & my && \\
\hline
t\_bdry & boundary decay time & 0.01 && \\
\hline
t\_Bbdry & boundary decay time for B & 0.01 && \\
\hline
eetop\_fraction & fraction old average energy & 1 & 0.01 & \\
                & at top boundary used in new &&& \\
\hline
htop & density scale height at top boundary & 0 && \\
\hline
rmin & minimum $\rho$ at top bounary = rmin*$<\rho>$ & 1.e-3 & 1e-2 & \\
\hline
rbot & fiducial densty at bottom boundary & -1 && \\
\hline
ebot & fiducial energy at bottom boundary & && \\
\hline
pbot & fiducial pressure at bottom boundary & && \\
\hline
B{x,y,z}0 & B at bottom boundary & 0 && \\
\hline
Binflow & impose B at bottome boundary & true && \\
\hline
t\_bdry & bounary decay time & 0.05 & 0.6 & \\
\hline
t\_Bbdry & boundry decay time for B & 0.01 && \\
\hline
t\_vbdry & boundary decay time for V inflow & 0 & 1.2 & \\
\hline
Uy\_bdry & smoothing transition from in to out flows & 0.01 && \\
\hline
uy\_max & limit velocity at top boundary & 20 & 2 & \\
\hline
pb\_fact & limit $\rho$ and $e$ perturbations due to B & 1 && \\
\hline
lb\_eampl & & 0 && \\
\hline

\end{tabular}
\end{center}

\begin{center}
{\Large Namelist slice}
\begin{tabular}{|l|l|c|c|c|}
\hline
name & description & default & atmosphere sun & turbulence  \\
\hline
do\_slice & write slices & false && \\
\hline
do\_vrms & write vrms instead of velocity & false && \\
\hline
tslice & time interval between slices& 1 && \\
\hline
ntslice && 10 && \\
\hline
nslice & timestep interval between slices & 1 && \\
\hline
jdir & normal to direction of slice & 3 && \\
\hline
jx,y,z && $(m{x,y,z}+1)/2$ && \\
\hline
nvar & number of slice variables & 1 && \\
\hline
var & variable number to make slice of & 0 && \\
\hline

\end{tabular}
\end{center}

\begin{center}
{\Large Namelist quench} \\
\begin{tabular}{|l|l|c|c|c|}
\hline
name & description & default & atmosphere sun & turbulence  \\
\hline
do\_quench & use quenching & false && t \\
\hline
qmax & maximum quenching & 8 && \\
\hline
qlim & limit second differences& 2 && 2 \\
\hline

\end{tabular}
\end{center}

\begin{center}
{\Large Namelist eqofst (combined EOS, Opacity table)}
\begin{tabular}{|l|l|c|c|c|}
\hline
name & description & default & atmosphere sun & turbulence  \\
\hline
do\_eos && true && \\
\hline
do\_ionization & calculate ionization & true && \\
\hline
do\_table & use table & false && \\
\hline
tablefile & table file of EOS and Opacity &&& \\
\hline

\end{tabular}
\end{center}

\begin{center}
{\Large Namelist eqofst (separate EOS, Opacity tables)}
\begin{tabular}{|l|l|c|c|c|}
\hline
name & description & default & atmosphere sun & turbulence  \\
\hline
do\_eos && true && \\
\hline
do\_ionization & calculate ionization & true && \\
\hline
do\_table & use table & false && \\
\hline
  eostabfile    & eos table file & EOSrhoe.tab && \\
\hline
  radtabfile    & opacity table file & kaprhoT.tab && \\
\hline
  do\_cubic\_eos  & interpolateion & true && \\
\hline
  do\_limit\_tab  & & false && \\
\hline
  verbose\_tab   & debugging & false && \\
\hline
  uur           & simulation to cgs units & 1.0e-7 && \\
\hline
  uul           & & 1.0e8 && \\
\hline
  uut           & & 1.0e2 && \\
\hline
  eelimMinE     & table limits & 1.0e-4 && \\
\hline
  eelimMaxE     & & 1.0e4 && \\
\hline
  rholimMinE    & & 1.0e-9 && \\
\hline
  rholimMaxE    & & 1.0e9 && \\
\hline
  ttlimMinR     & & 1.0e1 && \\
\hline
  ttlimMaxR     & & 1.0e7 && \\
\hline
  rholimMinR    & & 1.0e-9 && \\
\hline
  rholimMaxR    & & 1.0e9 && \\
\hline
  eelimE        & for backwards compatibility & 0.0 && \\
\hline
  rholimE       & & 0.0 && \\
\hline

\end{tabular}
\end{center}

\begin{center}
{\Large Namelist part} \\
\begin{tabular}{|l|l|c|c|c|}
\hline
name & description & default & atmosphere sun & turbulence  \\
\hline
do\_particles & trace particles & false && \\
\hline
fraction &&&& \\
\hline

\end{tabular}
\end{center}

The namelist /force/ may take different forms depending on the system being
modeled.  

Namenlist /init/ can be used to initialize a case.  

Namelist /expl/ is used when there are explosions.

Namelist cool specifies the whether there is cooling or not (do\_cool) and if so the variables
needed for a given type of cooling. 

\begin{center}
{\Large Namelist cool}
\begin{tabular}{|l|l|c|c|c|}
\hline
name & description & default & atmosphere sun & turbulence  \\
\hline
do\_cool & cool &  & t & f \\
\hline
intfile & &  && \\
\hline
nmu & number of rays & 0 & 0 2 & \\
\hline
nphi & number of azimuthal angles & 4 & 4 & \\
\hline
dphi & change in azimuthal angle each time step & 0 & 100 & \\
\hline
form\_factor & & 1 && \\
\hline
dtaumin & minimum $\Delta\tau$ & 0.1 && \\
\hline
dtaumax & maximum $\Delta\tau$  & 100 & 1e3 & \\
\hline
do\_newton & do newtonian cooling & false & t & \\
\hline
y\_newton & do Newtonian cooloing above & -0.3 & -0.4 & \\
\hline
dy\_newton & thickness trasnition zone & 0.05 && \\
\hline
t\_newton & timescale & 0.01 & 0.3 & \\
\hline
ee\_newton & fiducial energy & 5.265 && \\
\hline
ee\_min & minimum photospheric energy& 3.6 & 4.4 & \\
\hline
t\_ee\_min & timescale to raise to minimum & 0.005 & 0.003 & \\
\hline
do\_limb & & false && \\
\hline
mu0 & & 0 && \\
\hline
ny0 & & 0 && \\
\hline
mblocks & & 1 && \\
\hline
do\_fld & & false && \\
\hline
do\_conduction & & false && \\
\hline
do\_corona & & false && \\
\hline
do\_chromos & & false && \\
\hline
t\_chromos & & 1 && \\
\hline
ee\_chromos & & 7 && \\
\hline
do\_Casiana &  & false && \\
do\_top & & true && \\
\hline
r\_top & & 1.e-8 && \\
\hline
t\_top & & 1 && \\
\hline
ee\_top & damp fluctiations to ee\_top &  && \\
\hline
h\_top & transition for Newtonian cooling &  && \\
\hline
d\_top & & 2 && \\
\hline
do\_damp & & false && \\
\hline
t\_damp & & 1 && \\
\hline
iphot & & 1 && \\
\hline
ichrom & & 0 && \\
\hline
c\_scale &  & 1 && \\
\hline
do\_limit &  & false && \\
\hline
tt\_limit &  & 5e6 && \\
\hline
cdt\_cond &  & 0.05 && \\
\hline

\end{tabular}
\end{center}

A snapshot consists of the nine variables: density, 3 momenta, internal energy per
unit volume, temperature, 3 magnetic fields.  If a "from" file is specified in the io
namelist it is used to read an initial snapshot specifying all nine variables that
will be calculated evolving in time.  In addition, a mesh file must be selected
that gives the coordinate, coordinate spacing and Jacobian between phyical and
index spece at each grid location.  The first line are the three dimensions.  Then
for each dimension there is a line giving: the cell centered grid spacing, the face
centered grid spacing, the cell centered location, the face centered location, 
1/derivative of the cell centered locations with respect to the cell index,
1/derivative of the face centered locations with respect to the cell index.
If there is a "from" file, these values will be taken from the file from\_root.msh
if it exists.  Similarly a .tim file is sought with the time information.

Ouput consists of eleven files based on the root of the "file" file.  One is
"file" itself to which snapshots are written every nstep timesteps or tsnap time
intervals.  Another is a file of snapshots that overwrite each other every nscr
time steps or tscr time intervals.  These are direct access unformatted files. 
At the same interval as the saved snapshots are
written,  file root\_name.tim has the current time information added to it, a file 
of the various energy fluxes is writen to root\_name.flux and various
quatities are written to root\_name.stat.
A log file is written for each run.  The scrpt that starts starts the run begins it
by recording the date and time
of the start of the run, text describing the run, the size and date of the
executable, the number of cpus/node, the number of cores and a list of the cores.
As each namelist is read the value of
each parameter, whether default or read in from the namelists is
printed.  Next if a snapshot of the variables is read the name of the "from" file
is given, then the time, if a time file is found,  and then the first several values of each
variable near the top (lb) is printed as they are read in..
Every time step the log file is appended with the time step number, the time, time
interval and the location of the most restrictive of each of the courant conditions
due to viscosity, resistivity, density and energy changes.  Each time step a small 
text file root\_name.chk is also written that gives similar time step information.
At the start of each run a copy
of the input file is saved as well as added to a file of all the input files for
that run, a copy of the mesh file is saved, a file giving the
dimensions, grid spacing, number of variables and mpi decomposition is written.

